Backdoor Attack on Unpaired Medical Image-Text Foundation Models: A Pilot Study on MedCLIP

In recent years, foundation models (FMs) have solidified their role as cornerstone advancements in the deep learning domain. By extracting intricate patterns from vast datasets, these models consistently achieve state-of-the-art results across a spectrum of downstream tasks, all without necessitating extensive computational resources. Notably, MedCLIP, a vision-language contrastive learning-based medical FM, has been designed using unpaired image-text training. While the medical domain has often adopted unpaired training to amplify data, the exploration of potential security concerns linked to this approach hasn't kept pace with its practical usage. Notably, the augmentation capabilities inherent in unpaired training also indicate that minor label discrepancies can result in significant model deviations. In this study, we frame this label discrepancy as a backdoor attack problem. We further analyze its impact on medical FMs throughout the FM supply chain. Our evaluation primarily revolves around MedCLIP, emblematic of medical FM employing the unpaired strategy. We begin with an exploration of vulnerabilities in MedCLIP stemming from unpaired image-text matching, termed BadMatch. BadMatch is achieved using a modest set of wrongly labeled data. Subsequently, we disrupt MedCLIP's contrastive learning through BadDist-assisted BadMatch by introducing a Bad-Distance between the embeddings of clean and poisoned data. Additionally, combined with BadMatch and BadDist, the attacking pipeline consistently fends off backdoor assaults across diverse model designs, datasets, and triggers. Also, our findings reveal that current defense strategies are insufficient in detecting these latent threats in medical FMs' supply chains.

==> sections/algorithm.tex <==
\footnotetext[1]{$I$ and $T$ are unpaired.}

\begin{algorithm*}[ht]
    \caption{Our proposed backdoor methods for attacking MedCLIP}
    \label{alg:cap}
    \textbf{Notations: }\\{$img_i$: denotes the clean image and $\widetilde{img}_i$ denotes the poisoned image. \\ 
    $\lambda_1$, $\lambda_2$: two hyper-parameters to balance the strength the \textit{BadDist} loss. \\
    $sim(c,d)$: stands for the similarity between vector $c$ and $d$. \\
    $b$: batch size. $p$: embedding size.\\
    $\tilde{f}_{\theta}$: the poisoned MedCLIP $f_{\theta^{\star}}$ using our proposed method, where $\theta^{\star}$ is fixed whereas $\theta$ is learnable model parameters. \\
    $\mathcal{D}_{\rm sub}$: Subset sampled from MIMIC dataset to be poisoned for tuning poisoned MedCLIP $\tilde{f}_{\theta}$.\\
    $SM$: Semantic similarity matrix. $PM$: Predicted similarity matrix and it contains cosine similarity between image and text embeddings. See Sec.~\ref{method:overview} and Fig.~\ref{fig:framework}.\\
    $I$: Clean image labels within the training batch. $\widetilde{I}$: poisoned image labels.\\
    $T$: Text labels within the batch\footnotemark. $l$ is the labels as shown in Fig.~\ref{fig:framework}\\
    $\tau$: Temperature set as 0.07.\\
    $\mathcal{L}_{\rm SM}$: Semantic Matching Loss.\\
    %$ \alpha \otimes x$ stands for the proportion to poison a data point by a trade-off hyper-parameter $\alpha$.
    }
	\begin{algorithmic}[1]	
    \Procedure{\textbf{A}. BadDist} {$f_{\theta^{\star}}$, $\mathcal{D}_{\rm sub}$}:
    \Comment{See Sec.~\ref{method:baddist}}
    
    \State $\tilde{f}_{\theta}$ $\leftarrow$ Copy($f_{\theta^{\star}}$) \Comment{Deep copy the pre-trained MedCLIP}
    
        \For{$img_i$ in $\mathcal{D}_{\rm sub}$}
            % \State imgi $\leftarrow$ Backdoor(imgi) 
            % \Comment{poison img from different strategies} 
            
            \State $c_i \leftarrow f_{\theta^{\star}}(img_i)$
            
            \State $b_i \leftarrow f_{\theta^{\star}}(\widetilde{img}_i$)
            
            \State $c'_i \leftarrow \widetilde{f}_{\theta}(img_i)$
            
            \State $b'_i \leftarrow \widetilde{f}_{\theta}(\widetilde{img}_i$)
            
          \State $\mathcal{L}_{BadDist} = -\lambda_{1} \cdot \frac{\sum_{1}^p sim(c_i', c_i)}{p} + \lambda_2 \cdot \frac{\sum_{1}^psim(b_i', b_i)}{p}$ 
          
          \State $\theta$ $\gets$ $\mathop{\min}_{\theta} \mathcal{L}_{BadDist}$
          \Comment{Update the poisoned MedCLIP}
      \EndFor
      \textbf{return} $\tilde{f}_{\theta}$
\EndProcedure

\Procedure{\textbf{B} SenmaticMatchingLoss}{$f_{\theta}$, $I$, $T$}:
\Comment{See Sec.~\ref{method:semanticM} }
\State{$SM \leftarrow \frac{I \cdot T^T}{||I|| \cdot ||T||}$}\\

\State{$y_{mn}^{img \rightarrow txt} \gets \frac{exp SM_{mn}}{\sum_{n=1}^{b} exp SM_{mn}}$}
\Comment{Image to text soft targets}

\State{$y_{nm}^{txt \rightarrow img} \gets \frac{exp SM_{nm}}{\sum_{m=1}^{b} exp SM_{nm}}$}
\Comment{Text to image soft targets}\\

% \State{$PM \gets $}
\State{$\hat{y}_{mn} \gets \frac{exp PM_{nm} / \tau}{\sum_{m=1}^{b} exp PM_{nm} / \tau}$}
\Comment{Obtain predicted similarity with softmax}
\\

\State{$\mathcal{L}^{img \rightarrow l} \gets -\frac{1}{b}\sum_{m=1}^{b}\sum_{n=1}^{b} y_{mn} \log \hat{y}_{mn}$}

\State{$\mathcal{L}^{l \rightarrow img} \gets -\frac{1}{b}\sum_{n=1}^{b}\sum_{m=1}^{b} y_{nm} \log \hat{y}_{nm}$}

\State{$\mathcal{L}_{\textsc{\rm SM}} \gets \frac{\mathcal{L}^{img \rightarrow l} + \mathcal{L}^{l \rightarrow img}}{2}$}
\Comment{Semantic Matching Loss}

\State $\theta \gets \mathop{\min}_{\theta} \mathcal{L}_{\textsc{\rm SM}}$
          \Comment{Update the MedCLIP}
          
\State{\textbf{return} $f_{\theta}$}
\EndProcedure

\Procedure{\textbf{C}. poisonSenmaticMatrix} {$\tilde{f}_{\theta}$,$\widetilde{I}$, $T$}:
    % \For{ Sampling batches $img_i$, $img'_i$, $txt_i$, $txt'_i$ from $\mathcal{D}_{\rm sub}$ }
    %\Comment{Building Poisoned Dataset}
    % \State{$\widetilde{img}_i \stackrel{poison}{\longleftarrow} img_i$}
    % % \Comment{Inject trigger on image}
    % \State{$\widetilde{img'}_i \stackrel{flip}{\longleftarrow} img'_i$}
    % \Comment{Flip label for poisoned image}
    % \State{$\textsc{PoisonDataset} \leftarrow \textsc{PoisonDataset} \bigcup [(\widetilde{img_i}, \widetilde{img'_i}, txt_i, txt'_i)]$}
    % \EndFor
    % \For{txt in texts}
    % \State $[s_1, ...s_n] \leftarrow$ tokenized(txt)
    % \Comment{Sentence-level tokenization}
    % \For{$s_i$ in $[s_1, ...s_n]$}
    % \State $y_i \leftarrow$ ChexPert($s_i$)
    % \Comment{Label sentence}
    % \State $[(s_1, y_i), ... (s_n, y_n)] \leftarrow s_i, y_i$
    % \Comment{construct sentence-level pool}
    % \EndFor
    
    % \State $S \leftarrow S \bigcup [(s_1, y_1), ... (s_n, y_n)]$
    
    % \For{$img$, $txt$, $I$, $T$ in \textsc{PoisonDataset}}
    % \State{$b'_i \gets$ BackdoorCLIP($\widetilde{img_i}$)}
    % \Comment{Poison data with flipped label}
    % \State {$\widetilde{SM} \leftarrow \frac{I \cdot T^T}{||I|| \cdot ||T||}$}
    % \Comment{Poisoned Semantic Matrix}

    \State{$\widetilde{f}_{\theta} \gets \textsc{senmaticMatchingLoss}(\tilde{f}_{\theta}, \widetilde{I}, T)$}
    % \EndFor
    \Comment{Train MedCLIP with flipped label}
    \State{\textbf{return} $\tilde{f}_{\theta}$}
    \EndProcedure
        
	\end{algorithmic}
\end{algorithm*}
